Backward Responsibility in Transition Systems Beyond Safety

As the complexity of software systems rises, methods for explaining their behaviour are becoming ever-more important. When a system fails, it is critical to determine which of its components are responsible for this failure. Within the verification community, one approach uses graph games and Shapley values to ascribe a responsibility value to every state of a transition system. As this is done with respect to a specific failure, it is called backward responsibility. This paper provides tight complexity bounds for the computation of backward responsibility values for reachability, B\"uchi and parity objectives. For B\"uchi objectives, a polynomial algorithm is given to determine the set of responsible states, i.e. states with positive responsibility value. To analyse systems that are too large for standard methods, the paper presents a novel refinement algorithm that iteratively finds the set of responsible states. Several heuristics are proposed to guide the refinement algorithm. Its utility is demonstrated with a tool that implements refinement in addition to several other responsibility computation techniques.

==> fix-counter.tex <==
\makeatletter
\theoremstyle{definition}

% For some reason, the envcountsame option does not work for me, so this achieves the same thing (and ensures theorem-like environments do not have an italic body)

\newtheoremrep{theoremcopy}[theorem]{Theorem}

\let\case\relax
\let\c@case\relax
\spnewtheorem{case}[theorem]{Case}{\itshape}{\rmfamily}

\let\conjecture\relax
\let\c@conjecture\relax
\spnewtheorem{conjecture}[theorem]{Conjecture}{\itshape}{\rmfamily}

\let\corollary\relax
\let\c@corollary\relax
%\spnewtheorem{corollary}[theorem]{Corollary}{\bfseries}{\rmfamily}
\newtheoremrep{corollary}[theorem]{Corollary}

\let\definition\relax
\let\c@definition\relax
\spnewtheorem{definition}[theorem]{Definition}{\bfseries}{\rmfamily}

\let\example\relax
\let\c@example\relax
\spnewtheorem{example}[theorem]{Example}{\itshape}{\rmfamily}

\let\exercise\relax
\let\c@exercise\relax
\spnewtheorem{exercise}[theorem]{Exercise}{\itshape}{\rmfamily}

\let\lemma\relax
\let\c@lemma\relax
%\spnewtheorem{lemma}[theorem]{Lemma}{\bfseries}{\rmfamily}
\newtheoremrep{lemma}[theorem]{Lemma}

\let\note\relax
\let\c@note\relax
\spnewtheorem{note}[theorem]{Note}{\itshape}{\rmfamily}

\let\problem\relax
\let\c@problem\relax
\spnewtheorem{problem}[theorem]{Problem}{\itshape}{\rmfamily}

\let\property\relax
\let\c@property\relax
\spnewtheorem{property}[theorem]{Property}{\itshape}{\rmfamily}

\let\proposition\relax
\let\c@proposition\relax
%\spnewtheorem{proposition}[theorem]{Proposition}{\bfseries}{\rmfamily}
\newtheoremrep{proposition}[theorem]{Proposition}

\let\question\relax
\let\c@question\relax
\spnewtheorem{question}[theorem]{Question}{\itshape}{\rmfamily}

\let\solution\relax
\let\c@solution\relax
\spnewtheorem{solution}[theorem]{Solution}{\itshape}{\rmfamily}

\let\remark\relax
\let\c@remark\relax
\spnewtheorem{remark}[theorem]{Remark}{\itshape}{\rmfamily}

\makeatother
